Model Input Verification of Large Scale Simulations

Reliable simulations are critical for analyzing and understanding complex systems, but their accuracy depends on correct input data. Incorrect inputs such as invalid or out-of-range values, missing data, and format inconsistencies can cause simulation crashes or unnoticed result distortions, ultimately undermining the validity of the conclusions. This paper presents a methodology for verifying the validity of input data in simulations, a process we term model input verification (MIV). We implement this approach in FabGuard, a toolset that uses established data schema and validation tools for the specific needs of simulation modeling. We introduce a formalism for categorizing MIV patterns and offer a streamlined verification pipeline that integrates into existing simulation workflows. FabGuard's applicability is demonstrated across three diverse domains: conflict-driven migration, disaster evacuation, and disease spread models. We also explore the use of Large Language Models (LLMs) for automating constraint generation and inference. In a case study with a migration simulation, LLMs not only correctly inferred 22 out of 23 developer-defined constraints, but also identified errors in existing constraints and proposed new, valid constraints. Our evaluation demonstrates that MIV is feasible on large datasets, with FabGuard efficiently processing 12,000 input files in 140 seconds and maintaining consistent performance across varying file sizes.

==> introduction_old.tex <==
\section{Introduction}
% Introduction on the importance of simulations and in particular agent-based simulations.  

Agent-based modeling (ABM) has become an essential tool for simulating complex systems, offering insights into the dynamics of diverse and intricate networks.
ABS focuses on the interactions between individual agents, such as organisms, people, or artificial entities, within a system. This approach allows for the detailed examination of how collective behaviors and large-scale patterns emerge from the interactions of these agents. 
%Agent-based simulations are particularly valued for their ability to model diverse phenomena with varying degrees of complexity, providing researchers and policymakers with a dynamic tool to explore hypothetical scenarios, assess potential interventions, and make informed decisions. 

Recent advancements in computational power and data analytics have significantly broadened the applicability and importance of agent-based simulations (ABS).For example, in epidemiology, ABS have been pivotal in modeling the spread of infectious diseases, such as COVID-19 \cite{mahmood2022}, allowing for the exploration of various public health interventions and their potential impacts on disease transmission dynamics. Similarly, ABS provides a powerful framework for simulating the complex dynamics of forced migration, enabling the analysis of individual and collective behaviors under varying conditions and interventions \cite{suleimenova2017}. In environmental science, ABS have been used to simulate ecosystem interactions and biodiversity, providing insights into conservation strategies under changing climate conditions \cite{jahani2023}. 
%Likewise, in the realm of economics and social sciences, ABS have facilitated the exploration of market dynamics, social networks, and the emergence of collective behaviors from individual decision-making processes. 
The growing complexity and accessibility of ABS tools have not only expanded their application across traditional fields but have also made them instrumental in addressing some of the most pressing challenges of our time, from pandemic response to climate change mitigation.


%Furthermore, the integration of ABS with machine learning and big data has improved model fidelity and predictive capabilities, enabling simulations to incorporate real-time data for more precise outcomes. This synergy has not only broadened the use of ABS in traditional domains but has also positioned them as key players in addressing global challenges such as pandemic management and climate change mitigation, underscoring their growing importance in advancing our understanding of complex systems and aiding in strategic decision-making.

As simulation models increasingly influence decision-making  at multiple levels, establishing trust in these models becomes paramount. An important and often overlooked step in the process of model verification and validation is the fidelity of the input data. The initial conditions, parameters, and agent configurations contained within the input files form the bedrock upon which simulations are constructed. Ensuring the correctness of these inputs is not merely a preliminary step; it is a safeguard against the cascading effect that inaccuracies can have on the predictive power and reliability of the model’s output.


%Verification involves checking that the model has been correctly implemented according to its design, essentially ensuring that the model is built right. Validation, on the other hand, assesses whether the right model has been built by comparing its outputs with real-world data or phenomena, thereby ensuring the model's representational accuracy and predictive capabilities. 

%Input verification plays a pivotal role in the reliability of large-scale simulations.
%, which  are integral to fields ranging from engineering and physics to climate science and epidemiology. These simulations often depend on complex models that process vast amounts of data to predict future events, optimize systems, or explore hypothetical scenarios. Incorrect or poorly formatted input data can lead to misleading results, wasted resources, and potentially significant setbacks in research and development. 
By ensuring the accuracy, consistency, and validity of input files through rigorous verification processes, researchers and engineers can significantly reduce errors, enhance the simulation's fidelity, and make informed decisions based on trustworthy outcomes. 
%Consequently, input verification is not just a preliminary step but a fundamental aspect that underpins the integrity of large-scale simulation. 
Input verification can be seen as:
\begin{itemize}
    \item  A foundational step: it is the basis upon which the rest of the verification process is built. If inputs are incorrect, subsequent verification steps are undermined.
    \item A preventive measure: by detecting issues early, it prevents the propagation of errors through the simulation, saving time and resources.
    \item An enabler of reproducibility: correct and well-verified inputs are key to ensuring that simulations can be reliably replicated, which is a cornerstone of scientific research.
\end{itemize}

% Importance of verification and validations
% The role of input verification. What are the challenges and why existing approaches does not solve them 
% This work solves the abovementioned problems by streamlining the verification of input files. In particular, ... explain details about the tool. 
This paper presents an integrated approach to input verification, including schema validation for complex data structures and automated consistency checks for interconnected input files. We empirically validate the proposed verification toolset. Through evaluations conducted on existing projects, we demonstrate that the toolset has been proven to be  effective in identifying issues with input data within real-world simulation contexts. These findings shows the applicability of the toolset and its potential to  enhance the quality of simulation studies.

%{\bm Impact on Best Practices in Simulation Modeling}
Additionally, this work contributes to the evolution of best practices for conducting large-scale simulations. By streamlining input verification, it advocates for a paradigm shift within the simulation community towards methodologies that are both more robust and resistant to errors. The adoption of these practices is expected to improve the reliability, credibility and transparency of simulation outcomes.

The contributions of this paper are threefold:
\begin{itemize}
\item Toolchain Development: We present an automated toolchain specifically engineered for the validation of simulation input files, which streamlines the verification process. This toolchain not only checks for data consistency format correctness within single input files but also manages complex data-dependency constraints across multiple data dimensions and files.
\item Methodological framework: our contribution includes the establishment of a structured methodology that distills the best practices for input verification, fostering a disciplined approach to simulation setup. This framework ensures that the verification process is not only thorough but also repeatable, enhancing the quality and credibility of simulation results.
\item Requirements assessment: we have collected a set of  essential requirements in the form of exemplars that input verification tools must satisfy, catering to the complex nature of simulation data. This assessment lays down the foundational benchmarks that can drive the development of verification tools, ensuring they are equipped to handle the intricacies of real-world simulation scenarios.
\end{itemize}

\input{relatedwork}
\section{Tool Overview}

\input{formalism}
\input{overview}
\input{miv-seavea}
\input{exemplars}

\input{evaluation}

\input{llm}

\section{Discussion}
[braindump: We have demostrated diverse patterns, spanning simulation types and require different validation and verification patterns. It showcases that a multitenant approach is needed. ..]

\bibliographystyle{alpha}
\bibliography{miv}

\end{document}

==> microbenchmarks_old.tex <==

\subsection{Micorbenchmarks}
\label{lbl:microbench}
\begin{figure}[h]
\centering
\includegraphics[width=0.48\textwidth]{figures/microbenchmarks/benchmark_results_columns_per_file.png}
\includegraphics[width=0.48\textwidth]{figures/microbenchmarks/benchmark_results_data_complexity.png}
\includegraphics[width=0.48\textwidth]{figures/microbenchmarks/benchmark_results_num_files.png}
\includegraphics[width=0.48\textwidth]{figures/microbenchmarks/benchmark_results_rows_per_file.png}
\end{figure}

The FabGuard evaluation experiment was designed to assess the performance of this model input verification tool for large-scale simulations. The experiment utilized randomly generated tests and files to simulate various scenarios that FabGuard might encounter in real-world applications. The test files were generated with varying characteristics across four key dimensions: data complexity, number of columns per file, number of rows per file, and the total number of files processed.

Data complexity was measured on a scale from 1 to 10, with higher numbers representing more complex data structures. The number of columns per file ranged from 10 to 100, while the number of rows per file varied from 100 to 1000. To test scalability, the experiment processed between 1 and 100 files. For each configuration, the experiment measured two primary performance metrics: median execution time and median memory usage. %Mu runs were conducted for each configuration to ensure statistical significance of the results.

The microbenchmark results reveal consistent performance across various dimensions of input data, with no significant trends impacting scalability. Notably, FabGuard demonstrates consistent memory usage across different data complexities, numbers of columns, and rows per file. While slight variations in execution time were observed with changes in data complexity and file structure, these fluctuations were not substantial enough to significantly affect the tool's performance. The most notable relationship was a linear correlation between the number of files processed and execution time, suggesting predictable scaling for large-scale simulations. The absence of major performance bottlenecks across the tested parameters indicates that FabGuard can maintain consistent performance across a wide range of input scenarios.

\subsection{Micorbenchmarks Results}

The results of the FabGuard evaluation are presented in Figures 1-4, each focusing on a different aspect of the tool's performance:

%Figure \ref{fig:data_complexity} displays the relationship between data complexity and FabGuard's performance. The x-axis represents the data complexity scale from 1 to 10, while the y-axis shows the median execution time in seconds. A secondary y-axis represents the median memory usage in MB.

%Figure \ref{fig:columns_per_file} illustrates how the number of columns per file affects FabGuard's performance. The x-axis shows the number of columns ranging from 10 to 100, with the y-axis again representing median execution time and memory usage.

%Figure \ref{fig:rows_per_file} demonstrates the impact of the number of rows per file on FabGuard's performance. The x-axis displays the number of rows from 100 to 1000, with the y-axes showing execution time and memory usage as before.

%Figure \ref{fig:num_files} presents FabGuard's scalability in terms of the number of files processed. The x-axis shows the number of files from 1 to 100, while the y-axes represent execution time and memory usage.

Analysis of the experimental results reveals several key insights into FabGuard's performance characteristics:

\textbf{Data Complexity (Figure \ref{fig:data_complexity}):} FabGuard shows a slight upward trend in execution time as data complexity increases, but the relationship is not strongly linear. There is significant variability in execution times across different complexity levels, suggesting that other factors may influence performance more heavily. Notably, memory usage remains constant regardless of data complexity, indicating efficient memory management by FabGuard.

\textbf{Columns Per File (Figure \ref{fig:columns_per_file}):} As the number of columns per file increases, there is a general trend of increased execution time. However, this relationship is not strictly linear, and there are some fluctuations. This suggests that FabGuard's performance is somewhat sensitive to the number of columns, but the impact is moderate. Again, memory usage remains constant, demonstrating FabGuard's ability to handle varying numbers of columns without additional memory overhead.

\textbf{Rows Per File (Figure \ref{fig:rows_per_file}):} The relationship between the number of rows per file and execution time is non-linear, with noticeable peaks at 200, 600, and 900 rows. This pattern suggests that FabGuard's performance may be optimized for certain file sizes, with potential bottlenecks at specific row counts. The consistent memory usage across all row counts is a positive indication of FabGuard's efficient data handling.

\textbf{Number of Files (Figure \ref{fig:num_files}):} This dimension shows the most clear-cut relationship with FabGuard's performance. There is a strong linear correlation between the number of files processed and execution time, indicating that FabGuard scales linearly with the volume of files. This predictable scaling is a positive feature for large-scale simulations. The memory usage graph shows an interesting spike for a very small number of files, but quickly stabilizes, suggesting an initial overhead that becomes negligible as the number of files increases.

In conclusion, FabGuard demonstrates robust performance across various dimensions of input data. Its consistent memory usage is a standout feature, indicating efficient resource management. The tool's linear scalability with the number of files processed is particularly promising for large-scale applications. However, the non-linear relationship with the number of rows per file suggests an area for potential optimization. These insights can guide further development of FabGuard and inform best practices for its use in different scenarios.
